A Cookbook of 3D Vision: Data, Learning Paradigms, and Application

3D vision has rapidly evolved, driven by increasingly diverse data representations, learning paradigms, and modeling strategies. Yet the field remains fragmented across representations and benchmarks, making it difficult to develop unified perspectives on efficiency, fidelity, and scalability. This work provides a data-centric taxonomy of 3D vision that connects geometric representations, datasets, learning frameworks, and applications within a single conceptual map. We begin by analysing the principal structural representations of 3D data--point clouds, meshes, voxels, and 3D Gaussians--along with their acquisition pipelines. We then examine how dataset design, benchmark construction, and supervision regimes shape recent advances, spanning 2D-supervised 3D learning, implicit neural representations, and 4D world modeling. Through this integrative lens, we clarify the relationships among representations, learning paradigms, and downstream tasks in reconstruction, generation, and video modeling, offering a consolidated view of emerging trends toward balancing efficiency and fidelity and toward multimodal geometric grounding.

==> sections/20-problems.tex <==
\section{Problem Landscape in 3D Vision }
\label{sec:landscape}

The field of 3D vision encompasses a diverse set of tasks aimed at perceiving, reconstructing, and understanding the three-dimensional structure of the world from visual data. These tasks vary widely in terms of their objectives, input modalities (e.g., single or multi-view RGB images, depth maps, LiDAR scans, or point clouds), and output formats (e.g., depth maps, voxel grids, meshes, or neural radiance fields). To provide a clear and structured overview of this landscape, we categorize 3D vision problems into several major groups: geometry estimation, 3D reconstruction, scene understanding, cross-modal generation, and scene understanding. Each category contains a range of well-studied and emerging problems, such as depth estimation, point cloud segmentation, NeRF-based modeling, and BEV perception. This section aims to systematically define and organize these core tasks, setting the foundation for our subsequent discussion of traditional and learning-based methods.

\subsection{Geometry Estimation}

\paragraph{Monocular Depth Estimation.}
Monocular Depth Estimation is the task of predicting the depth (distance from the camera) of each pixel in a scene using a single RGB image. It is an inherently ill-posed problem, as many different 3D scenes can produce the same 2D projection.

Multi-view Geometry-Based Methods can be solved by using multiple images using spatial relationship of multiple images. Traditional methods such as Structure from Motion(SFM)\cite{wang2023visualgeometrygroundeddeep}, Stereo Matching, Multi-View Stereo (MVS). However, it all have defect and heavily rely on some thing like camera pose. Since 2014, deep learning method try to reconstruct the depth map by one picture.  CNN/Transformer-based monocular methods allow depth prediction from a single image, enabling fast, real-time applications.\cite{eigen2014depthmappredictionsingle}  \cite{godard2019diggingselfsupervisedmonoculardepth}
\cite{ranftl2021visiontransformersdenseprediction}

\paragraph{6D Object Pose Estimation.}

\paragraph{Surface Normal Estimation.}
\paragraph{Camera Pose Estimation.}

\paragraph{Multi-view Geometry.}

\subsection{3D Reconstruction}

\paragraph{Multi-view Stereo (MVS).}
\paragraph{Single-view 3D Reconstruction.}
\paragraph{Point Cloud Reconstruction.}
\paragraph{Volumetric Reconstruction.}
\paragraph{Surface Mesh Reconstruction.}
\paragraph{Implicit Reconstruction.}
\paragraph{Neural Radiance Fields (NeRF and Variants).}

\subsection{Understanding}

\paragraph{Point Cloud Classification.}
\paragraph{3D Object Detection.}
\paragraph{3D Semantic Segmentation.}
\paragraph{3D Instance Segmentation.}
\paragraph{3D Part Segmentation.}
\paragraph{3D Human Pose Estimation.}
\paragraph{Shape Retrieval.}

\subsection{Multimodal \& Generation}

\paragraph{RGB-D Fusion.}
\paragraph{Image-to-Point Cloud Generation.}
\paragraph{Text-to-3D Generation.}
\paragraph{Image/Video-to-3D Generation.}
\paragraph{3D-aware GANs.}
\paragraph{NeRF Editing and Generation.}
\paragraph{Multimodal Representation Learning.}

\subsection{Scene Understanding}

\paragraph{Simultaneous Localization and Mapping (SLAM).}
\paragraph{3D Scene Parsing.}
\paragraph{Indoor Scene Reconstruction.}
\paragraph{Bird's Eye View (BEV) Perception.}
\paragraph{Occupancy Mapping.}
\paragraph{3D Panoptic Segmentation.}
\paragraph{3D Scene Graph Generation.}

==> sections/40-model_based_approach.tex <==
\section{3D Geometric Foundation model Learning Paradigms and Applications}


\textcolor{red}{This section, 3D rendering paradigms and applications should be separately discussed. First discuss 3D rendering paradigm, then discuss applications.}



Modern 3D vision has increasingly shifted from explicit geometry pipelines toward learned systems that couple representation design, supervision, and downstream applications~\cite{kato2020differentiablerenderingsurvey,wang2024dust3r,trellis}. This section reviews the main learning paradigms behind modern 3D reconstruction, generation, and geometry-aware video modeling. We begin with differentiable rendering, then move to image-aligned reconstruction frameworks, and finally discuss how these ideas extend to 4D generation and embodied world models.



\subsection{Preliminary: Differentialble Rendering}

Early learning-based 3D methods often relied on direct 3D supervision, where losses such as Chamfer distance, Earth Mover's Distance, or volumetric TSDF errors were computed explicitly in 3D space~\cite{fan2016pointsetgenerationnetwork,qi2017pointnet,qi2017pointnetpp,wu2015shapenets,choy20163dr2n2unifiedapproachsingle}. Although conceptually simple, these objectives become computationally prohibitive for dense voxels or high-resolution surfaces. A pivotal transition came from differentiable rendering frameworks (e.g., Neural Mesh Renderer, Soft Rasterizer, OpenDR)~\cite{kato2017neural3dmeshrenderer,liu2019softrasterizerdifferentiablerenderer,10.1007/978-3-319-10584-0_11}. By backpropagating through the image formation process, these methods replace explicit 3D supervision with image-plane losses on color, depth, or silhouettes:
\[
\mathcal{L}_{\mathrm{photo}} = \sum_{i=1}^N \big\| I_i - \mathcal{R}(\mathcal{M}_\theta, P_i) \big\|^2
\]
where $\mathcal{R}$ is the differentiable rendering operator, $\mathcal{M}_\theta$ is the 3D representation, and $P_i$ denotes the camera parameters~\cite{Differentiable rendering:}. The evolution of this rendering operator defines the computational limits of 3D learning:
\begin{itemize}
    \item \textbf{Volume Rendering (NeRFs):} Early continuous frameworks utilized ray-marching and volumetric integration. While physically principled, the dense multi-layer perceptron (MLP) queries along each ray made end-to-end training on high-resolution data computationally prohibitive~\cite{gao2025nerfneuralradiancefield}.
    \item \textbf{Tile-based Rasterization (3DGS):} The introduction of 3D Gaussian Splatting revolutionized the rendering bridge. By replacing implicit MLPs with explicit 3D Gaussians and utilizing a highly optimized, differentiable $\alpha$-blending rasterizer, 3DGS reduced rendering times from seconds to milliseconds. This breakthrough directly enabled the training of massive, feed-forward 3D foundation models~\cite{kerbl20233dgaussiansplattingrealtime}.
\end{itemize}

\subsection{3D Reconstruction}

3D reconstruction seeks to recover object or scene geometry from one or more images. Classical pipelines build on local features such as SIFT and SURF~\cite{790410,BAY2008346}, estimate cameras with Structure-from-Motion (SfM)~\cite{560851,schoenberger2016sfm,10.1007/978-3-030-37629-1_37}, and densify geometry with multi-view stereo or point-cloud fusion~\cite{Furu:2010:PMVS,schoenberger2016mvs}. These pipelines remain geometrically principled, but they are only weakly end-to-end trainable and often degrade under sparse views, weak texture, or strong appearance change.

Neural methods changed the bottleneck from camera solving to representation design: the central question is now how to predict dense 3D structure while keeping supervision and memory costs tractable. This motivates image-aligned point maps, rays, and other per-pixel 3D outputs that preserve dense geometry without resorting to dense voxel losses~\cite{wang2024dust3r,wang2025vggtvisualgeometrygrounded,depthanything3}.

\subsubsection{Image-Aligned Point Clouds \& Rays}

A leading direction in modern reconstruction is Image-aligned point-map and ray-based representations because they preserve dense per-pixel structure while keeping learning and supervision in the image domain~\cite{wang2024dust3r,wang2025vggtvisualgeometrygrounded,depthanything3}.

\begin{itemize}
    \item \textbf{DUSt3R~\cite{wang2024dust3r}:} DUSt3R predicts dense point maps, so each image pixel is associated with a 3D coordinate. Instead of relying on explicit multi-view optimization at training time, it learns through confidence-weighted regression on image-aligned 3D outputs. A simplified form of the objective is:
    \begin{equation}
        \mathcal{L}_{\mathrm{pmap}} = \sum_i \left( \| C_i \odot (P_i - P^*_i) \| - \alpha \log C_i \right)
    \end{equation}
    where $P_i$ and $P^*_i$ are the predicted and ground-truth 3D points, and $C_i$ models aleatoric uncertainty.

    \item \textbf{VGGT (Visual Geometry Grounded Transformer)~\cite{wang2025vggtvisualgeometrygrounded}:} VGGT scales the image-aligned paradigm to large multi-view sets by jointly predicting cameras, point maps, depth maps, and point tracks with a shared transformer backbone. A representative multi-task objective is:
    \begin{equation}
        \mathcal{L}_{\mathrm{total}} = \mathcal{L}_{\mathrm{camera}} + \mathcal{L}_{\mathrm{depth}} + \mathcal{L}_{\mathrm{pmap}} + \lambda \mathcal{L}_{\mathrm{track}}
    \end{equation}
    This joint formulation yields a reusable geometric backbone for downstream 3D, 4D, and embodied reasoning tasks.

    \item \textbf{RayZer~\cite{jiang2025rayzerselfsupervisedlargeview}:} RayZer studies self-supervised novel view synthesis from unposed, uncalibrated image collections. It factorizes the input into camera and scene representations and trains entirely through 2D reconstruction, without explicit 3D supervision:
    \begin{equation}
        \mathcal{L}_{\mathrm{RayZer}} = \| \hat{I}_{\mathrm{target}}(\hat{P}_{\mathrm{target}}) - I_{\mathrm{target}} \|_2^2
    \end{equation}
    By penalizing rendered-view mismatch under self-predicted poses, RayZer encourages a geometry-aware latent space even in the absence of calibration.

    \item \textbf{$\pi^3$~\cite{wang2025pi3scalablepermutationequivariantvisual}:} $\pi^3$ removes the dependence on a fixed reference view by enforcing permutation-equivariant supervision over unordered image sets. Rather than regressing a single global coordinate frame, it optimizes local point maps and relative poses:
    \begin{equation}
        \mathcal{L}_{\pi^3} = \mathcal{L}_{\mathrm{local}}(X_i, X^*_i) + \mathcal{L}_{\mathrm{relative}}(T_{i \to j}, T^*_{i \to j})
    \end{equation}
    Here $X_i$ denotes a scale-invariant local point map and $T_{i \to j}$ an affine-invariant relative pose. This design improves robustness to input ordering and scales better to large, unordered view sets.

    \item \textbf{Depth Anything 3~\cite{depthanything3}:} Built on top of DINOv2 features~\cite{oquab2023dinov2}, DA3 predicts both a depth map $D$ and a per-pixel ray tensor $R \in \mathbb{R}^{H \times W \times 6}$ whose channels encode ray origin and direction. Its supervision can be summarized as:
    \begin{equation}
        \mathcal{L}_{\mathrm{DA3}} = \mathcal{L}_{\mathrm{depth}}(D, D^*) + \mathcal{L}_{\mathrm{ray}}(R, R^*)
    \end{equation}
    where $R = (O, V)$. By collapsing multiple geometric heads into a depth-plus-ray representation, DA3 unifies single-image, multi-view, and video-space recovery within one prediction format.
\end{itemize}

% \paragraph{Ecosystem Extensions and Spatiotemporal Dynamics.}
% These image-aligned backbones have quickly produced a broader family of follow-up models. MASt3R recasts matching as a 3D-constrained problem, while MUSt3R and SLAM3R adapt the same paradigm to symmetric multi-view alignment and online tracking~\cite{wang2024dust3r,leroy2024mast3r,cabon2025must3r,liu2024slam3r}. For monocular reconstruction, MoGe and MoGe-2 separate relative geometry from absolute scale and use large visual priors to recover metric point maps from single images~\cite{wang2025mogeunlockingaccuratemonocular,wang2025moge2}.

% A parallel branch pushes these ideas from point maps toward directly renderable Gaussian scenes. MV-DUSt3R+ compresses sparse-view reconstruction into a single feed-forward stage, Splatt3R lifts unposed image pairs into Gaussian splats, and NoPoSplat and PF3plat further remove explicit pose supervision for sparse image collections by jointly recovering camera geometry and splat parameters~\cite{tang2024mvdust3rsinglestagescenereconstruction,smart2024splatt3rzeroshotgaussiansplatting,ye2024poseproblemsurprisinglysimple,hong2025pf3platposefreefeedforward3d}. Together, these methods narrow the gap between image-aligned geometry backbones and render-ready 3D Gaussian outputs.

% The same line of work is now being extended from offline batches to long or streaming sequences. StreamVGGT replaces global attention with causal processing and an implicit KV cache, IncVGGT controls history growth with view fusion and pruning, and VGG-T$^3$ compresses geometry state through test-time training rather than explicit caching~\cite{wang2025vggtvisualgeometrygrounded,su2026xstreamvggtextremelymemoryefficientstreaming,fang2025incvggt,elflein2026vggt3offlinefeedforward3d}.

% For dynamic scenes, Easi3R and VGGT4D extract motion cues from pretrained geometry transformers without expensive retraining, while 4D-VGGT, Flow4R, and MonST3R model geometry and motion jointly with native spatiotemporal prediction~\cite{chen2025easi3restimatingdisentangledmotion,hu2025vggt4d,wang2025_4dvggt,qian2026flow4runifying4dreconstruction,zhang2025monst3rsimpleapproachestimating}. iGGT further couples geometric consistency with semantic learning, enabling instance-level outputs that connect reconstruction backbones to VLM and VLA pipelines~\cite{li2025iggtinstancegroundedgeometrytransformer}.

\subsection{3D Generation}

3D content generation aims to synthesize faithful and controllable assets from text, images, or sparse visual cues. Recent progress can be organized into four broad paradigms: optimization against 2D priors, feed-forward multi-view reconstruction, native 3D latent modeling, and scene-level generation~\cite{dreamfusion,shi2024mvdreammultiviewdiffusion3d,lrm,trellis,chen2025sam3d}.

\paragraph{Optimization via 2D Generative Priors:}
Early text-to-3D systems circumvented the scarcity of labeled 3D data by distilling pretrained 2D diffusion priors into a 3D representation. DreamFusion and Magic3D optimize NeRF-like fields through Score Distillation Sampling (SDS), while Make-It-3D, Latent-NeRF, and DreamGaussian improve efficiency or geometric fidelity by changing the underlying representation~\cite{dreamfusion,magic3d,makeit3d,Latent-nerf,tang2024dreamgaussiangenerativegaussiansplatting}. These optimization-based pipelines remain flexible, but they are typically slow and prone to oversmoothing or inconsistent multi-view geometry.

\paragraph{Feed-Forward Multi-View Reconstruction:}
To avoid per-prompt optimization, later work adopted a synthesis-then-reconstruction pipeline. Multi-view diffusion models such as MVDream and Zero-1-to-3 first generate view-consistent images, and large reconstruction models (LRMs) then map these images directly into 3D assets~\cite{shi2024mvdreammultiviewdiffusion3d,zero123,lrm}. Representative systems include InstantMesh, MeshFormer, and Hunyuan3D 2.0/2.5, which recover meshes, tri-planes, or Gaussian-like representations in seconds rather than minutes~\cite{instantmesh,meshformer,Hunyuan3D2.0,Hunyuan3D2.5}.

Recent mesh-centric variants further push this pipeline toward directly usable surfaces. MeshGPT autoregressively models triangle meshes, Progressive Rendering Distillation adapts large 2D diffusion priors for instant text-to-mesh synthesis, and CraftsMan3D combines native 3D generation with a geometry refiner for high-fidelity mesh outputs~\cite{Siddiqui_2024_CVPR,Ma_2025_CVPR,craftsman3d}.

\paragraph{Native 3D Foundation Models \& Structured Latents:}
More recent work models 3D content directly in native latent spaces rather than treating 3D as a proxy target for 2D diffusion. TRELLIS learns structured 3D latents that can be decoded into radiance fields, 3D Gaussians, or meshes, whereas \textbf{SAM 3D} formulates 3D reconstruction as large-scale \textbf{Rectified Conditional Flow Matching (RCFM)} with separate geometry and texture modules~\cite{trellis,chen2025sam3d}. A core contribution of SAM 3D is breaking the \textbf{3D "data barrier"} through a multi-stage training framework—comprising synthetic pretraining, semi-synthetic mid-training, and real-world alignment—powered by a \textbf{Model-in-the-Loop (MITL)} data engine. This engine enables human annotators to verify and align 3D assets at unprecedented scale, resulting in a foundation model capable of lifting any object in a single image into composable 3D assets (meshes or 3D Gaussian splats). These models point toward reusable 3D foundation backbones that support both generation and reconstruction.

\paragraph{Scene-Level Generation:}
Beyond single objects, scene generation increasingly emphasizes composition, layout, and editability. 3D-SceneDreamer enforces 3D consistency in text-driven scene synthesis, while AnyHome targets open-vocabulary generation of structured indoor homes with explicit room- and object-level organization~\cite{Zhang_2024_CVPR,fu2024anyhomeopenvocabularygenerationstructured}. This trend broadens 3D generation from isolated assets to coherent, navigable environments.

\subsection{The Synergy of Reconstruction and Generation}

Historically, 3D reconstruction and 3D generation were treated as separate tasks. Recent work increasingly couples them: generative priors fill missing geometry, and explicit reconstruction signals stabilize open-ended generation~\cite{chen2025sam3d,shi2024mvdreammultiviewdiffusion3d,wang2024dust3r,wang2025vggtvisualgeometrygrounded,depthanything3,trellis}.

\paragraph{Generation for Reconstruction (Generative Priors for Ill-posed Geometry):}
Single-view and sparse-view reconstruction are ill-posed because multiple 3D explanations can match the same observations. Generative approaches address this ambiguity by imposing strong priors over shape and texture. \textbf{SAM 3D} is a primary example, using RCFM to predict per-object geometry and texture from single-view context~\cite{chen2025sam3d}. Similarly, diffusion-assisted reconstruction pipelines use MVDream or Zero-1-to-3 to synthesize missing viewpoints before an LRM-style reconstructor lifts them into 3D~\cite{shi2024mvdreammultiviewdiffusion3d,zero123,lrm}.

\paragraph{Reconstruction for Generation (Geometric Grounding for Controllability):}
Conversely, purely generative 3D pipelines often suffer from geometry drift, duplicated structures, or weak scale control. Reconstruction backbones such as DUSt3R, VGGT, and DA3 provide point maps, cameras, depth, and rays that can be injected as explicit structure into downstream generative models~\cite{wang2024dust3r,wang2025vggtvisualgeometrygrounded,depthanything3}. Their role is not to hallucinate content, but to constrain generation to physically consistent 3D layouts.

\paragraph{Unified Latent Spaces and the Data Flywheel:}
The deeper convergence appears in shared latent spaces. TRELLIS and SAM 3D both suggest that a common structured latent can support synthesis, decoding, and geometric extraction within one system~\cite{trellis,chen2025sam3d}. Such shared spaces also enable a \textbf{data flywheel}: generative models expand synthetic 3D corpora, while reconstruction models convert large image or video collections into additional 3D supervision for the next training round~\cite{wang2024dust3r,chen2025sam3d}. \textbf{SAM 3D} makes this virtuous cycle explicit through its MITL pipeline, where model outputs are human-vetted to create new supervision~\cite{chen2025sam3d}. MegaSynth similarly shows that large-scale synthesized scenes can be used to pretrain reconstruction systems and improve scene-level generalization~\cite{Jiang_2025_CVPR}.

\subsubsection{Geometric Regulation in Video Diffusion Models}

Large video diffusion models (VDMs) achieve strong visual quality, but they still struggle to preserve stable 3D geometry across time and camera motion~\cite{hong2022cogvideo,yang2024cogvideox,wan2025}. Recent work therefore injects geometric priors directly into video generation, either through explicit 3D modeling, geometry-aware supervision, or structured controls~\cite{bahmani20233dawarevideogeneration,zhang2024worldconsistentvideodiffusionexplicit,wu2025geometryforcingmarryingvideo}. We group these strategies into three representative paradigms:

\begin{itemize}
    \item \textbf{Geometric Preference Alignment:} This line of work treats geometry as a reward or preference signal rather than modifying the core VDM architecture. Epipolar-DPO measures pairwise epipolar consistency through quantities such as the fundamental matrix and Sampson distance, then uses those signals for preference optimization~\cite{kupyn2025epipolargeometryimprovesvideo}. VideoGPA follows a similar idea by distilling dense geometric preferences from pretrained geometry models and applying DPO to suppress physically implausible videos~\cite{du2026videogpadistillinggeometrypriors}.

    \item \textbf{Feature-Level Geometry Forcing:} Here, 3D structure is injected into the latent features of the diffusion model. Geometry Forcing aligns video diffusion features with depth-aware or reconstruction-driven 3D representations during denoising~\cite{wu2025geometryforcingmarryingvideo}. Related work on epipolar attention restricts cross-view interactions to epipolar lines derived from camera geometry, reducing view inconsistency and structural hallucination~\cite{tseng2023consistentviewsynthesisposeguided}.

    \item \textbf{3D-Aware Control Mechanisms:} Instead of conditioning only on 2D signals such as edges or poses, this paradigm uses explicit 3D inputs to steer generation. Diffusion as Shader (DaS) conditions on dense 3D trajectories extracted from point clouds or depth, turning video synthesis into a geometry-guided, rendering-like process with finer spatial control~\cite{gu2025diffusionshader3dawarevideo}.
\end{itemize}

\subsection{From 3D to 4D and Embodied World Models}

The scope of 3D vision is expanding from static shape recovery to temporally persistent scene understanding and action-conditioned simulation. Three directions are especially important: dynamic rendering, 3D-native world models, and spatially grounded embodied reasoning.

\paragraph{4D Rendering and Spatiotemporal Representations:}
Static 3D representations are poorly suited to non-rigid motion and topology changes. Dynamic 3D Gaussians and 4D Gaussian Splatting extend splat-based rendering with temporal state or deformation fields, enabling real-time rendering of dynamic scenes while maintaining cross-view consistency~\cite{luiten2023dynamic3dgaussianstracking,wu20244dgaussiansplattingrealtime}. By making time a first-class variable, these methods represent motion as structured 3D evolution rather than as a sequence of unrelated 2D frames. On the generation side, SV4D and SV4D 2.0 emphasize multi-frame and multi-view consistency for dynamic content, while CAT4D combines multi-view video diffusion with deformable 3D Gaussian reconstruction, further blurring the line between 4D generation and 4D recovery~\cite{xie2025sv4ddynamic3dcontent,yao2025sv4d20enhancingspatiotemporal,wu2024cat4dcreate4dmultiview}.

\paragraph{3D-Native World Models:}
Whereas 4D rendering reconstructs observed motion, world models aim to predict future states and support planning. Earlier approaches mostly relied on latent 2D rollouts or generic sequence modeling~\cite{hafner2020dreamcontrollearningbehaviors,micheli2023transformerssampleefficientworldmodels,hansen2024tdmpc2scalablerobustworld}. More recent systems such as PointWorld and ParticleFormer move the state space into persistent 3D points or particles, making manipulation and physical interaction easier to simulate and control~\cite{huang2026pointworldscaling3dworld,huang2025particleformer3dpointcloud}. Navigation World Models extends this trend to embodied navigation, while WorldSimBench highlights that evaluating such systems requires more than visual realism; temporal consistency, action relevance, and simulator faithfulness also matter~\cite{bar2025navigationworldmodels,qin2024worldsimbenchvideogenerationmodels}. At a larger scale, platforms such as Cosmos indicate how world modeling is being framed as a foundation-model problem for physical AI~\cite{nvidia2025cosmosworldfoundationmodel}.

\paragraph{Spatial Intelligence in Vision-Language-Action (3D-VLA):}
The practical value of 3D-native world models lies in embodied interaction. Instead of mapping image tokens directly to embodiment-specific motor outputs, recent systems increasingly ground perception, language, and control in a shared 3D scene representation~\cite{10.5555/3692070.3692890,hong20233dllm,xu2023pointllm,huang2026pointworldscaling3dworld}. This shift improves viewpoint robustness, enables richer spatial reasoning, and makes action policies less dependent on a single camera or robot embodiment.

